Faceting for direction-dependent spectral deconvolution

The new generation of radio interferometers is characterized by high sensitivity, wide fields of view and large fractional bandwidth. To synthesize the deepest images enabled by the high dynamic range of these instruments requires us to take into account the direction-dependent Jones matrices, while estimating the spectral properties of the sky in the imaging and deconvolution algorithms. In this paper we discuss and implement a wide-band wide-field spectral deconvolution framework (DDFacet) based on image plane faceting, that takes into account generic direction-dependent effects. Specifically, we present a wide-field co-planar faceting scheme, and discuss the various effects that need to be taken into account to solve for the deconvolution problem (image plane normalization, position-dependent PSF, etc). We discuss two wide-band spectral deconvolution algorithms based on hybrid matching pursuit and sub-space optimisation respectively. A few interesting technical features incorporated in our imager are discussed, including baseline dependent averaging, which has the effect of improving computing efficiency. The version of DDFacet presented here can account for any externally defined Jones matrices and/or beam patterns.

==> AlgoDegrid.tex <==
 for ThisVis in VisSet:
   u,v,w,t_i,nu_i=ThisVis.coord
   p,q=ThisVis.pq
   for ThisFacet in ListFacet:
      Dp=Jones[p][t_i][nu_i]
      Dp=Jones[p][t_i][nu_i]
    li,mi=ThisFacet.


==> NCPReview.tex <==

\section{NonCoplanar Facetting}

\subsection{First order correction}

Another way to do (approximate) coplanar faceting is to consider
taking the phase error in Equation 4.19 into account while gridding
the facets. One such strategy to include w per gridded visibility is
to Taylor expand the term to a first order approximation around the
original phase center. The first order approximation leads to a
remarkable transformation for u and v as pointed out by \citet{Kogan09}.
Specifically, $\Delta n_i$ can be written as:

\begin{alignat}{2}
\label{eq:dni}
\Delta n_i=&
\sqrt{1-\l^2+\m^2}-\sqrt{1-\l_i^2+\m_i^2}\\
\approx&-\frac{1}{\sqrt{1-\l_i^2+\m_i^2}}\left(
\l_i\Delta \l_i+\m_i\Delta \m_i
\right)
\label{eq:dni_approx0}
\end{alignat}

\noindent which has the remarkable property to be equivalent to a
coordinate change in $uv$-coordinates:

\begin{alignat}{2}
\label{eq:Kogan}
\exp{
\left(-2 i\pi \frac{\nu}{c}
\vec{b}_{pq,t}^T
\vec{\Delta s}\right)}\sim&
\exp{
\left(-2 i\pi \frac{\nu}{c}
(u'\Delta l_i+
v'\Delta m_i)
\right)}\\
\textrm{with }
u'=u-w\frac{\l_i}{\sqrt{1-\l_i^2+\m_i^2}}\\
\textrm{and }
v'=v-w\frac{\m_i}{\sqrt{1-\l_i^2+\m_i^2}}
\end{alignat}

The linear approximation of $\Delta n_i$ (Eq. \ref{eq:dni}) by the
relation in Eq. \ref{eq:dni_approx0} is plotted in
Fig. \ref{fig:Comparison}.


\subsection{W-projection extention}

A better approximation is:

\begin{alignat}{2}
\Delta n_i=&
\sqrt{1-\l^2+\m^2}-\sqrt{1-\l_i^2+\m_i^2}\\
\approx&-\frac{1}{\sqrt{1-\l_i^2+\m_i^2}}\left(
\l_i\Delta \l_i+\m_i\Delta \m_i
\right)\\
&+\sqrt{1-\Delta \l_i^2-\Delta \m_i^2}\\
\label{eq:dni_approx1}
\end{alignat}

\noindent and that is plotted too in Fig. \ref{fig:Comparison}. The
right hand term of Eq. \ref{eq:dni_approx1} $\left(\sqrt{1-\Delta
  \l_i^2-\Delta \m_i^2}\right)$ becomes a classical w-projection
kernel $\mathcal{W}$ that
can be used to grid/degrid the data:

\begin{alignat}{2}
\mathcal{W}\left(\Delta \l_i,\Delta \m_i\right)=&
\exp{
\left(-2 i\pi \frac{\nu}{c}w
\left(\sqrt{1-\Delta
  \l_i^2-\Delta \m_i^2}\right)
\right)}
\end{alignat}

It has the great advantage to be
axisymetric for using 1-dimentional convolution functions.


==> PolStokes.tex <==

\section{Stokes parameters}

\begin{alignat}{2}
\textbf{X}_{\vec{s}}=& 
\begin{bmatrix}
\EXp\EXq^* & \EXp\EYq^*\\
\EYp\EXq^* & \EYp\EYq^*
\end{bmatrix}
\end{alignat}

\noindent and is connected to the astrophysically-relevent Stokes parameters I (total
intensity), Q and U (linear polarisation) and V (circular
polarisation) \citep[see][for details]{Oleg11}. We can write somthig
like \textbf{[please check, this should be wrong for the V-stokes]}:

\def\I{\textrm{I}}
\def\Q{\textrm{Q}}
\def\U{\textrm{U}}
\def\V{\textrm{V}}

\begin{alignat}{2}
\textbf{X}_{\vec{s}}=& 
\begin{bmatrix}
I+Q & U-iV\\
U+iV & I-Q
\end{bmatrix}/2
\end{alignat}

In general, Q, U and V are zeros so $\textbf{X}_{\vec{s}}$ is scalar matrix.


==> SSD_algo2.tex <==
\def\ComplicatedLine{
\argmin{\vec{\pi_{i}}}
\left\|
\DirtyVecNorm-\widetilde{\TransferFunc_{\phi_i}}\vec{\pi_i}
\right\|_{\bm{Q}}
}

\def\ResidVis{
\Vis-\bm{\mathcal{A}}\displaystyle\sum_{i} \bm{\Pi^i}\widehat{\vec{\pi_i}}
}

\begin{algorithm}[t!]
\SetAlgoLined
 \KwData{$\DirtyVecNorm$, $t$, $\alpha$}
 \KwResult{
The estimate $\widehat{\vec{\pi}}$ of
$\vec{\pi}$ in the basis function $\mathcal{P}$.}
initialization: $\widehat{\vec{\pi}}=\vec{0}$\;
 \While{$\max{\{\DirtyVecNorm\}}>t$}{
   \tcc{Find location of brightest pixel:} $i=\argmax{}\left(\DirtyVecNorm\right)$\;
  %$\widehat{\vec{\overline{x}_{B,i}}}=\argmin{\vec{\overline{x}_{B,i}}}{\widetilde{\TransferFunc_{\phi}}\vec{\overline{x}_{B,i}}}$\;
   Find locally best sky model centered on pixel $i$: $\widehat{\vec{\pi_{i}}}=\ComplicatedLine$\;
  $\widehat{\vec{\pi}}\leftarrow
   \widehat{\vec{\pi}}+\alpha\ \widehat{\vec{\pi_i}}$\;
  $\DirtyVecNorm\leftarrow\DirtyVecNorm-\widetilde{\TransferFunc_{\phi_{i}}}\widehat{\vec{\pi_i}}$\;
  %% \eIf{understand}{
  %%  go to next section\;
  %%  current section becomes this one\;
  %%  }{
  %%  go back to the beginning of current section\;
  %% }
   
 }
 $\DirtyVecNorm =\bm{\mathcal{A}}^H
 \bm{\mathcal{W}} \left(\ResidVis\right)$

 \caption{\SSDCLEAN/ deconvolution algorithm}
\end{algorithm}


